Graph Augmentation for Recommendation

Graph augmentation with contrastive learning has gained significant attention in the field of recommendation systems due to its ability to learn expressive user representations, even when labeled data is limited. However, directly applying existing GCL models to real-world recommendation environments poses challenges. There are two primary issues to address. Firstly, the lack of consideration for data noise in contrastive learning can result in noisy self-supervised signals, leading to degraded performance. Secondly, many existing GCL approaches rely on graph neural network (GNN) architectures, which can suffer from over-smoothing problems due to non-adaptive message passing. To address these challenges, we propose a principled framework called GraphAug. This framework introduces a robust data augmentor that generates denoised self-supervised signals, enhancing recommender systems. The GraphAug framework incorporates a graph information bottleneck (GIB)-regularized augmentation paradigm, which automatically distills informative self-supervision information and adaptively adjusts contrastive view generation. Through rigorous experimentation on real-world datasets, we thoroughly assessed the performance of our novel GraphAug model. The outcomes consistently unveil its superiority over existing baseline methods. The source code for our model is publicly available at: https://github.com/HKUDS/GraphAug.

==> intro2.tex <==
\section{Introduction}
\label{sec:intro}

In recent years, Graph Neural Networks (GNNs) have emerged as powerful frameworks for Collaborative Filtering (CF), due to its capacity to capture high-order relationships among users and items~\cite{gao2022survey,wang2019neural,he2020lightgcn}. Yet, most of GNN-based methods are designed with supervised settings, which requires sufficient training labels for producing accurate representations. To reduce the dependency on supervision labels, Self-Supervised Learning (SSL) provides a good data augmentation paradigm to empower recommenders with pretext task~\cite{yu2022self}. These works exploit rich unlabeled user behavior data to extract informative knowledge as augmented data~\cite{yu2021socially}. 

Among many self-supervised learning methods, Graph Contrastive Learning (GCL) methods~\cite{wu2021self,xia2022hypergraph,lin2022improving} become the dominant research line and provide state-of-the-art recommendation performance, by building contrastive data augmentation schemes upon graph neural architectures. Following the mutual information maximization principle, the essence of GCL is ``comparing'' the generated augmented views, which maximizes the consistency between encoded embeddings from the positive pairs and pushes away the representations of negative samples~\cite{zhu2021graph}. SGL~\cite{wu2021self} is the first attempt to build GCL-based CF model, which randomly omits a set of user-item interaction edges to generate corrupted graph structures. In analogy to SGL, mostly recent works (\eg, NCL~\cite{lin2022improving}, HCCF~\cite{xia2022hypergraph}) focus on establishing contrastive views from subgraph embeddings based on their manually-designed information aggregators.


Due to the inherent design of GCL, its success of data augmentation for user preference learning, is largely relied on the quality of the contrastive embeddings learned from the augmented graph structural views. However, real-world recommendation environments usually contain interaction noise, due to the diversity and randomness of user behaviors, such as misclicks~\cite{tian2022learning} and popularity bias~\cite{chen2021autodebias}. Most existing GCL methods performing augmentation with noisy information, are likely to provide inaccurate self-supervised learning signals, which misleads the recommender to understand user preference well. To be specific, randomly perturbing the graph structures~\cite{wu2021self,yu2022graph} will cause the information loss of important interaction patterns for many long-tail items~\cite{liu2020long,zhang2021model}, which heavily deteriorates the recommendation performance. 



